Not Just Pretty Pictures: Toward Interventional Data Augmentation Using Text-to-Image Generators

Neural image classifiers are known to undergo severe performance degradation when exposed to inputs that are sampled from environmental conditions that differ from their training data. Given the recent progress in Text-to-Image (T2I) generation, a natural question is how modern T2I generators can be used to simulate arbitrary interventions over such environmental factors in order to augment training data and improve the robustness of downstream classifiers. We experiment across a diverse collection of benchmarks in single domain generalization (SDG) and reducing reliance on spurious features (RRSF), ablating across key dimensions of T2I generation, including interventional prompting strategies, conditioning mechanisms, and post-hoc filtering. Our extensive empirical findings demonstrate that modern T2I generators like Stable Diffusion can indeed be used as a powerful interventional data augmentation mechanism, outperforming previously state-of-the-art data augmentation techniques regardless of how each dimension is configured.

==> figures/NICO_Vis_1.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{ICLR2024/image_new/nico_1_sbs_2.png}
    \caption{\textbf{NICO++ SDG Performance.} Single Domain Generalization (SDG) OfficeHome result in comparison with baselines (dash lines) and OURS (solid lines) using ResNet-18 (Left) and ResNet-50 (Right). The number reported follows format in \cref{fig:PACS_1}.}
    \label{fig:Officehome_1}
\end{figure}

==> figures/Officehome_Vis_1.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{ICLR2024/image_new/officehome_1_sbs_2.png}
    \caption{\textbf{OfficeHome SDG Performance.} Single Domain Generalization (SDG) OfficeHome result in comparison with baselines (dash lines) and OURS (solid lines) using ResNet-18 (Left) and ResNet-50 (Right). The number reported follows format in \cref{fig:PACS_1}.}
    \label{fig:Officehome_1}
\end{figure}

==> figures/PACS_Vis_1.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{ICLR2024/image_new/pacs_1_sbs_2.png}
    \caption{\textbf{PACS SDG Performance.} Single Domain Generalization (SDG) PACS result in comparison with baselines (dash lines) and OURS (solid lines) using ResNet-18 (Left) and ResNet-50 (Right). Accuracies reported are the average test accuracy of the three remaining target domains when training using the indicated source domain on each axis. The average performance is reported numerically in legend.}
    \label{fig:PACS_1}
\end{figure}

==> figures/SCM.tex <==
% \begin{figure}[t]
%   \centering
%     %\includegraphics[width=0.65\linewidth]{./images/SCM.png}
%    \includegraphics[width=0.65\linewidth]{./images/fig2redone.png}
%     \caption{Structural Causal Model (SCM) defined in \cite{AugmentationIntervention} to represent the data generation process, where shaded nodes and white nodes denote observed and unobserved variables, respectively. Given environmental factors $\mathbf{c}$ and labels $y$ where $\mathbf{c}$ and $y$ may be spuriously correlated through a confounder $s$, generated images $\mathbf{x}$ are dependent on environmental features $h_{\mathbf{c}}$ and causal features $h_{y}$. Our goal is to approximate interventions (indicated as the hammer) on $\mathbf{c}$.}
%    \label{fig:scm}
% \end{figure}


%\begin{wrapfigure}{r}{0.5\textwidth}
% \vspace{-3mm}
%  \centering
 % \includegraphics[width=0.48\textwidth]{./images/SCM.png}
 % \caption{Structural Causal Model (SCM) defined in \cite{AugmentationIntervention} to represent the data generation process, where shaded nodes and white nodes denote observed and unobserved variables, respectively. Given environmental factors $\mathbf{c}$ and labels $y$ where $\mathbf{c}$ and $y$ may be spuriously correlated through a confounder $s$, generated images $\mathbf{x}$ are dependent on environmental features $h_{\mathbf{c}}$ and causal features $h_{y}$. Our goal is to approximate interventions (indicated as the hammer) on $\mathbf{c}$.}
 % \label{fig:scm}
  % \vspace{-8mm}
%\end{wrapfigure}

